MLExpert: Towards a Generalist Agentic Model for Autonomous Machine Learning Engineering

Large language models (LLMs) are expanding from assisting scientific research and engineering to autonomously developing and improving AI systems, advancing AI for AI (AI4AI) as a pathway toward recursive self-improvement (RSI). Workflow-driven machine learning engineering (MLE) systems provide a practical path toward this pursuit through complex orchestration that manages long-horizon experimentation, while recent MLE systems adopt model-directed interaction, allowing models to autonomously organize experiments and adapt optimization strategies based on execution feedback. However, feedback from each experiment reflects several preceding decisions, and a long MLE run contains many such costly experiments. Training must therefore select useful supervision from long interaction trajectories and learn from intermediate outcomes. We propose a post-training method for autonomous long-horizon MLE optimization and apply it to train MLExpert, a 35B Mixture-of-Experts agentic model. We design the Kaggle-MLE Factory to construct executable tasks and an interaction harness for model-directed experimentation. Hierarchical agentic SFT transfers general tool-use and coding capabilities to MLE through outcome-guided supervision. Windowed Interaction RL (WIRL) treats the multi-turn decisions between successive experiment results as an execution window and assigns it a shared outcome-based reward. Asynchronous collection and policy correction support policy updates before the trajectory ends. On MLE-Bench Lite, MLExpert improves the average medal rate of the base model from 37.9% to 72.7%, achieving performance comparable to larger frontier models such as Kimi-K3 and GLM-5.3. Further experiments show that MLExpert improves performance on NatureBench Lite, agent scaffold optimization, and algorithm optimization, suggesting that the learned optimization capability generalizes to other tasks.

==> section/8_statements.tex <==
%% 两项声明均不计入正文页数限制。
%% AI use statement 为 required，Reproducibility statement 为 recommended。

\subsection*{AI use statement}

We used large language models to assist with manuscript translation and
language editing, as well as experimental code implementation. The authors
reviewed and revised the assisted text and code and take responsibility for
the final content of this work.

\subsection*{Reproducibility statement}

Task construction is described in Section~\ref{sec:kaggle_factory} and
Appendix~\ref{app:kaggle_factory}. Training methods and key hyperparameters
are detailed in Sections~\ref{sec:hierarchical_sft} and~\ref{sec:wirl} and
Appendix~\ref{app:posttraining_details}. Evaluation protocols and detailed
benchmark results are provided in Section~\ref{sec:exp_setup} and
Appendix~\ref{app:experiment_details}. The \sname{} model weights are publicly
available at \url{https://huggingface.co/InternScience/M1}.

